Self-Supervised Speech Representations are More Phonetic than Semantic

Self-supervised speech models (S3Ms) have become an effective backbone for speech applications. Various analyses suggest that S3Ms encode linguistic properties. In this work, we seek a more fine-grained analysis of the word-level linguistic properties encoded in S3Ms. Specifically, we curate a novel dataset of near homophone (phonetically similar) and synonym (semantically similar) word pairs and measure the similarities between S3M word representation pairs. Our study reveals that S3M representations consistently and significantly exhibit more phonetic than semantic similarity. Further, we question whether widely used intent classification datasets such as Fluent Speech Commands and Snips Smartlights are adequate for measuring semantic abilities. Our simple baseline, using only the word identity, surpasses S3M-based models. This corroborates our findings and suggests that high scores on these datasets do not necessarily guarantee the presence of semantic content.

==> figures/hubert-large-slice.tex <==
\begin{figure}[h]
    \centering
    \vspace{-1em}
    \includegraphics[width=0.45\textwidth]{figures/hubert-slice.pdf}
    \caption{
        Word representations of HuBERT-large.
        Unlike \Cref{fig:hubert-large}, feature slicing is used instead of audio slicing.
    }
    \label{fig:hubert-large-slice}
\end{figure}


==> figures/wav2vec2-large.tex <==
\begin{figure}[h]
    \centering
    \vspace{-1em}
    \includegraphics[width=0.45\textwidth]{figures/w2v2.pdf}
    \caption{
        Word representations of wav2vec 2.0-large, audio slicing and average pooling is used.
    }
    \label{fig:wav2vec2-large}
\end{figure} 


==> sections/9_shinji_checklist.tex <==
\section{Paper writing TIPS}

\subsection{Acknowledgements}
\begin{itemize}
    \item (v) Please ask all your co-authors (especially supervisors) whether they need them.
    \item (v) In the double-blind case, it is not allowed in the submission stage, but please recover this information for the camera-ready submission.
    \item (v) If you use PSC/NCSA, please add the following: Experiments of this work used the Bridges2 system at PSC and Delta system at NCSA through allocations CIS210014 and IRI120008P from the Advanced Cyberinfrastructure Coordination Ecosystem: Services \& Support (ACCESS) program, supported by National Science Foundation grants \#2138259, \#:2138286, \#:2138307, \#:2137603, and \#:2138296.
\end{itemize}

\subsection{As a coauthor}
\begin{itemize}
    \item (x) As co-authors, we have to be responsible for the entire contents of the paper. Please check the paper carefully. Also, at least check this TIPS and give the authors appropriate advice.
    
\end{itemize}

\subsection{When you get comments}
\begin{itemize}
    \item (ongoing) Try to reflect all comments. If they point out something wrong or their points are based on misunderstanding, which is still your fault. Some of your documents just confuse them. Please make sure to fix them.
    \item (ongoing) If someone points out some issues, please ensure that these points may be applied to the other parts of the document. When they point out one issue, please try fixing all related parts in the entire document.
\end{itemize}

\subsection{Main documents}
\begin{itemize}
    \item (v) Long sentences (say more than three lines) must be split. \red{This might be too strict in interspeech format, so I allowed 4 lines in some cases.}
    \item (v) When you want to excuse something or describe something, which breaks logic a little bit, use a footnote. This is a very useful technique (See footnote 4 in the reference paper).
    \item (v) When you have an important message, try to emphasize it in different sections like abstract, intro, experiments, etc. It is okay to rephrase and be redundant in the message as reviewers might not read every section in detail, but still, they have to get the message.
    \item (v) Try to make the paper concise: some parts can be safely removed when they are isolated with the main message of the paper and the following discussion (See equation (14) in the reference paper).
    \item () Include as many back-pointers (i.e., refer to previous content such as equation number or section number when discussing new stuff. Basically, we should have \label and \ref as many as possible) in the paper as possible. Those help you to make each section of the paper tighter and reduce the difficulty for others reading your paper (See Sections 2 and 5 in the reference paper).
    \item (v) make the paper structured. It is difficult for non-native English readers to read the long plain text. Please use the section structure, itemize/enumerate, etc.
\end{itemize}

\subsection{Abbreviations}
\begin{itemize}
    \item (v) Add definitions when they appear first. (even for trivial words like HMM, ASR)
    \item () Add some back-pointer when using them so that the reader can easily go back to check the definition.
\end{itemize}

\subsection{Related works}
\begin{itemize}
    \item () Provide an explicit distinction from the prior studies. Please always finalize each paragraph with how they are different from the proposed method explicitly (See Section 4 in the reference paper).
\end{itemize}

\subsection{Equations (x)}
\begin{itemize}
    \item () Equations are like figures. This makes the paper look more scientific. Please try to put basic equations even if you think it is trivial
    \item () Use algorithm.sty to describe the algorithm. This also makes the paper look more scientific
    \item () Do not duplicate the same characters for different variables.
    \item () Distinguish the type of variables/values (e.g., scalar ($x$), vector ($\mathbf{x}$), matrix ($\mathbf{X}$), the sequence ($X$). Please check the mathematical notation (page xi and xii) in Bishop's PRML
    \item () Add the domain when you introduce a new variable, e.g., $X = (\mathbf{x}_t \in \mathbb{R}^D | t=1, \cdots, T)$ with the explanation, e.g., $X$ is a $T$-length sequence of $D$-dimensional speech features.
    \item () When you want to distinguish some variable with some descriptions, use superscript with the non-italic font (e.g., cross entropy loss $\mathcal{L}^{ce} \rightarrow \mathcal{L}^\text{ce}$
    \item () Some operations must be non-italic (e.g., $max() \rightarrow \text{max}()$
    \item () We should not only list the equations. We should add some discussions. Avoid paragraph breaks after equations.
    \item () Equations must not have any mistakes.
\end{itemize}

\subsection{Grammar check}
\begin{itemize}
    \item (v) Use some auto-grammar checks (I'm using Grammarly Pro)
    \item (v) Use a Google translator to convert your English to your 1st language and check if it is reasonably translated.
\end{itemize}

\subsection{Tables and Figures}
\begin{itemize}
    \item (v) Do not simply copy the figure from other papers (including your previous papers). It breaks the copyright and also gives the reviewer a very negative impression.
    \item (v) Make Tables and Figures self-consistent. For example, add a brief experimental design and sometimes brief discussions in the caption.
    \item (v) If it uses some abbreviations, also explain the abbreviation even if it is described in the main body or other tables \& figures.
    \item () Try to put figures and tables on the bottom or top of the page and avoid including them in the middle of the document as much as possible, but there can be exceptions.
    \item () Wherever possible in figures, refer to respective variables in equations and be consistent with the notation (See Table 5 in the reference paper).
    \item (x) Try to categorize the table entries and use \texttt{\\hline} to separate them when the table is complex. For example, do not put the Oracle numbers and your numbers in the same category.
    \item () Provide some visualizations or examples for the AI/ML/NLP conferences (See Table 4 and Figure 3 in the reference paper).
    \item (v) Check the figures to be colorblind-friendly / black-and-white-friendly. 
\end{itemize}

\subsection{Experimental discussions}
\begin{itemize}
    \item (x) Please be careful about the decimal place, e.g., 14.05 and 13.1 $\rightarrow$ 14.05 and 13.10 or 14.1 (or 14.0) and 13.1
   \item (v) Try to make a story and a message. It's not interesting to read plain descriptions of the experimental results without them. We don't need details, but some overall trends to get the message.
   \item () Try to make connections between different paragraphs/subsections in the discussion by using \texttt{ref{}} or \texttt{eqref{}}
   \item (v) When many experiments are presented, explaining each experiment's results is a good idea instead of discussing the experimental settings and results separately.
   \item (v) If your experiments are worse than those of the other reports, please emphasize the excuse (e.g., footnote or other clear remarks in the table/figure). The reviewers often missed the detailed conditions and judged only on the numbers. If there are clear remarks, we can avoid such misjudgments.
\end{itemize}

\subsection{References}
\begin{itemize}
    \item (v) Try to list more than 25 references (more references give the impression that this paper performs a good survey in this area)
    \item (v) Put balanced references across several research groups. Reviewers who are assigned to one paper are usually from different institutes.
    \item (v) It is very good to cite your (or your colleagues') papers to increase your and your colleagues' visibility! Also, it is a good way to show that we are experts in this field (However, this logic cannot be used for the double-blind case)
    \item (v) but be careful about the above balance issue, and always try to include competitors' references (e.g., EEND and TS-VAD).
    \item () Please clean up/normalize the reference. If you simply paste the reference from Google Scholar BibTex, it would include a lot of noises
    \item () be careful about the capitalization in the title of the BibTeX, e.g., HMM should be {HMM}.
    \item () cite the published version instead of the arXiv version or Wikipedia (why? They are not reviewed. They may include some mistakes!).
    \item () Use “et al.” for more than XXX numbers of authors if you want to save space.
\end{itemize}
